Multi-Cell Coordinated Beamforming for Integrate Communication and Multi-TMT Localization

This paper investigates integrated localization and communication in a multi-cell system and proposes a coordinated beamforming algorithm to enhance target localization accuracy while preserving communication performance. Within this integrated sensing and communication (ISAC) system, the Cramer-Rao lower bound (CRLB) is adopted to quantify the accuracy of target localization, with its closed-form expression derived for the first time. It is shown that the nuisance parameters can be disregarded without impacting the CRLB of time of arrival (TOA)-based target localization. Capitalizing on the derived CRLB, we formulate a nonconvex coordinated beamforming problem to minimize the CRLB while satisfying signal-to-interference-plus-noise ratio (SINR) constraints in communication. To facilitate the development of solution, we reformulate the original problem into a more tractable form and solve it through semi-definite programming (SDP). Notably, we show that the proposed algorithm can always obtain rank-one global optimal solutions under mild conditions. Finally, numerical results demonstrate the superiority of the proposed algorithm over benchmark algorithms and reveal the performance trade-off between localization accuracy and communication SINR.

==> subText/hybrid.tex <==
\section{Hybrid Beamforming Algorithm to Solve the Problem \eqref{eq:problem_hybrid}}
In this section, we propose a hybrid beamforming algorithm to address
problem \eqref{eq:problem_hybrid}. When compared to digital beamforming, hybrid beamforming
offers advantages in terms of lower hardware costs and power consumption, 
making it more suitable for practical implementation. However, 
the complexity of solving the hybrid beamforming algorithm increases due to the additional 
constant modulus constraints imposed on the phase shifters and the non-convex SINR constraints.
A common approach to the hybrid beamforming algorithm involves solving problem \eqref{eq:problem_hybrid} 
by approximating the optimal digital beamformer. This is achieved by first obtaining the 
optimal digital beamformer, followed by designing the hybrid beamformer to minimize the 
Euclidean distance between the digital and hybrid beamformer. However, 
this method does not guarantee satisfaction of the SINR constraints, 
which could potentially lead to performance degradation.
Therefore, we propose a novel hybrid beamforming algorithm that directly solves the problem \eqref{eq:problem_hybrid}
by alternating direction method of multipliers (ADMM) \cite{boydDistributedOptimizationStatistical2010}.

Similar to the digital beamforming algorithm, we introduce two auxiliary variables, i.e., $\mu_1$ and $\mu_2$, 
to transform the fractional structure of the SINR constraints into matrix inequalities.
Besides, we introduce two sets of auxiliary variables, i.e., $\left\{\mathbf{t}_{1,1}, \ldots,\mathbf{t}_{1,K}, \ldots,
\mathbf{t}_{M,1}, \ldots,\mathbf{t}_{M,K}\right\}$ and 
$\left\{{q}_{1},{q}_{2},\ldots,{q}_{M}\right\}$, to make the problem 
\eqref{eq:problem_hybrid} more tractable. 
Then, we can rewrite the problem \eqref{eq:problem_hybrid} as follows:
\begin{subequations}
	\begin{align}
		\ \ \ \  & \min_{\left\{\mathbf{F}_{RF,m}, \mathbf{f}_{BB,m, k},
		\mathbf{t}_{m, k}, q_m, \mu_1, \mu_2\right\}} 
		\mu_1+\mu_2 \\
		\text { s.t. } &  \sum_{m=1}^M \sum_{k=1}^K \left\| \mathbf{t}_{m, k}  \right\|^2   \leq P   \\
		& \sum_{k=1}^K \left\| \mathbf{t}_{m, k}  \right\|^2   \leq P_m, \forall m   \\
		&SINR_{m,k} \left( \left\{ \mathbf{t}_{m, k} \right\} \right) \geq \Gamma, \forall m, k \\
		&\left[\begin{array}{cc}
			\mathbf{\Lambda Z} \mathbf{\Lambda}^T & \mathbf{e}_i \\
			\mathbf{e}_i^T & \mu_i
		\end{array}\right] \succeq 0, i=1,2 \\
		&\mathbf{t}_{m,k}=\mathbf{F}_{RF,m}\mathbf{f}_{BB,m,k}, \forall m,k \\
		&{q}_{m}=\mathbf{a}^T\left( \theta_m \right) \left( \sum_{k=1}^{K} \mathbf{t}_{m,k} \mathbf{t}_{m,k}^H \right)
				\mathbf{a}^*\left( \theta_m \right), \forall m
	\end{align} 
	\label{eq:problem_hybrid_lmi}
\end{subequations}
Correspondingly, the equation \eqref{J_ele} can be rewritten as:
\begin{equation}
	\begin{aligned}
		J(\tau_{m,n},\tau_{m,n}) & = \frac{8\pi^2 L \beta^2 \left| \varepsilon_{m,n} \right|^2}{\sigma_s^2}
		\\ & \times q(m)  \mathbf{a}^T\left(\theta_m\right) 
		\mathbf{a}^{\star}\left(\theta_m\right)  
	\end{aligned}  \label{J_ele3}
\end{equation}
Placing the equality constraints in \eqref{eq:problem_hybrid_lmi} into the objective function, 
yielding the augmented Lagrangian function:
\begin{equation}
	\begin{aligned}
		\hspace{-0.8cm}\mathcal{L} & = \mu_1  +  \mu_2  \\ 
		& \! + \! \frac{\rho_{1}}{2} \sum_{m=1}^{M} \sum_{k=1}^{K}   
		\left\| \mathbf{t}_{m,k}-\mathbf{F}_{RF,m}\mathbf{f}_{BB,m,k} + \mathbf{d}_{m,k} \right\|^2   \\
		& \! + \! \frac{\rho_2}{2} \! \sum_{m=1}^{M}\! \left| q_m \! - \! \mathbf{a}^T\left( \theta_m \right) \!
		\left( \! \sum_{k=1}^{K} \mathbf{t}_{m,k} \mathbf{t}_{m,k}^H \! \right)\!
		\mathbf{a}^*\left( \theta_m \right)\! + \! b_m \right|^2 
	\end{aligned}  \label{aug_lag}
\end{equation}
where $\left\{ \mathbf{d}_{1,1}, \ldots, \mathbf{d}_{1,K}, \ldots, \mathbf{d}_{M,1}, \ldots, \mathbf{d}_{M,K}  \right\}$
and $\left\{ b_1, b_2, \ldots, b_M \right\}$ are the dual variables associated with the equality constraints, 
and $\rho_1$ and $\rho_2$ are the penalty parameters.
According to the ADMM framework \cite{boydDistributedOptimizationStatistical2010}, 
we split the optimization problem  into the following five subproblems:
\begin{itemize}
	\item \textbf{Subproblem 1:} Update $\left\{\mathbf{t}_{m,k}\right\}$
	by minimizing the augmented Lagrangian function \eqref{aug_lag} with respect to $\left\{\mathbf{t}_{m,k}\right\}$
	while fixing $\left\{\mathbf{F}_{RF,m}\right\}$, $\left\{\mathbf{f}_{BB,m,k}\right\} $, $\left\{q_m\right\}$,
	$\left\{\mathbf{d}_{m,k}\right\} $, $\left\{ b_m\right\} $,
	$\mu_1$, and $\mu_2$.
	\item \textbf{Subproblem 2:} Update $\left\{q_m\right\}$, $\mu_1$, and $\mu_2$
	by minimizing the augmented Lagrangian function \eqref{aug_lag} with respect to $\left\{q_m\right\}$, $\mu_1$, and $\mu_2$
	while fixing $\left\{\mathbf{F}_{RF,m}\right\}$, $\left\{\mathbf{f}_{BB,m,k}\right\} $, 
	$\left\{\mathbf{d}_{m,k}\right\} $ and $\left\{ b_m \right\}$.
	\item \textbf{Subproblem 3:} Update $\left\{\mathbf{f}_{BB,m,k}\right\}$ by minimizing the augmented Lagrangian function 
	\eqref{aug_lag} with respect to $\left\{\mathbf{f}_{BB,m,k}\right\}$ while fixing $\left\{\mathbf{F}_{RF,m}\right\}$, 
	$\left\{q_m\right\}$,$\left\{\mathbf{d}_{m,k}\right\} $, $\left\{ b_m\right\} $,
	$\mu_1$, and $\mu_2$.
	\item \textbf{Subproblem 4:} Update $\left\{\mathbf{F}_{RF,m}\right\}$ by minimizing the augmented Lagrangian function 
	\eqref{aug_lag} with respect to $\left\{\mathbf{F}_{RF,m}\right\}$ while fixing $\left\{\mathbf{f}_{BB,m,k}\right\}$, 
	$\left\{q_m\right\}$,$\left\{\mathbf{d}_{m,k}\right\} $, $\left\{ b_m \right\}$,
	$\mu_1$, and $\mu_2$.
	\item \textbf{Subproblem 5:} Update the auxiliary variables $\left\{\mathbf{d}_{m,k}\right\}$ and $\left\{b_m\right\}$.
\end{itemize}
The ADMM algorithm iterates over these subproblems until convergence is achieved.
In the following, we provide the detailed solution to each subproblem at the $\left(i+1\right)$-th iteration.
\subsection{Subproblem 1: Update $\left\{\mathbf{t}_{m,k}\right\}$}
The subproblem 1 can be formulated as:
\begin{subequations}
	\begin{align}
		& \min_{\left\{\mathbf{t}_{m,k}\right\}}  
		\frac{\rho_1}{2} \sum_{m=1}^{M} \left| q_m  \right. \nonumber \\
		& - \left. \mathbf{a}^T\left( \theta_m \right) 
		\left(\sum_{k=1}^{K} \mathbf{t}_{m,k} \mathbf{t}_{m,k}^H \right) \mathbf{a}^*\left( \theta_m \right)  
		+  b_m \right|^2 \nonumber  \label{27a}\\ 
		&   + \frac{\rho_{2}}{2} \sum_{m=1}^{M} \sum_{k=1}^{K} 
		\left\| \mathbf{t}_{m,k}-\mathbf{F}_{RF,m}\mathbf{f}_{BB,m,k} + \mathbf{d}_{m,k}
		\right\|^2   \\
		\text { s.t. } & \sum_{m=1}^{M} \sum_{k=1}^{K} \left\| \mathbf{t}_{m,k} \right\|^2   \leq P \\
		& SINR_{m,k} \left( \left\{ \mathbf{t}_{m,k} \right\} \right) \geq \Gamma, \forall m, k
	\end{align}  \label{sub1}
\end{subequations}
This subproblem presents a non-convex optimization challenge, 
as evidenced by both the objective function and the SINR constraints. 
The complexity is particularly heightened due to the inclusion of a quartic term 
in the objective function, which poses significant difficulties in problem handling.

In order to address this subproblem, 
we redefine $\mathbf{t}_{m}$ as a transposed vector, 
specifically:
\begin{equation}
	\mathbf{t}_{m} = \left[ \mathbf{t}_{m,1}^T,\mathbf{t}_{m,2}^T, \ldots, 
		\mathbf{t}_{m,K}^T \right]^T
\end{equation}
Following this redefinition, we can accordingly reformulate 
the constraints for total power and per BS power:
\begin{equation}
	\begin{aligned}
		\sum_{m=1}^{M}  \mathbf{t}_{m}^H  \mathbf{t}_{m}  \leq P
	\end{aligned} \label{sub1_4}
\end{equation}
\begin{equation}
	\begin{aligned}
		\mathbf{t}_{m}^H  \mathbf{t}_{m}  \leq P_{m}, \forall m
	\end{aligned} \label{sub1_42}
\end{equation}
Correspondingly, the SINR constraint can be rewritten as:
\begin{equation}
	\begin{aligned}
		\left\|\left[\mathbf{H}_{m, k} \mathbf{t} ; \sigma_n\right]\right\|^2
		\leq\left(1+\frac{1}{\Gamma}\right)\left|\mathbf{s}_{m, k}^H \mathbf{H}_{m, k} \mathbf{t}\right|^2, \forall m, k
	\end{aligned} \label{sub1_2}
\end{equation}
where:
\begin{equation}
	\mathbf{H}_{m, k}=\operatorname{diag}\left\{\mathbf{H}_{1, m, k}, \mathbf{H}_{2, m, k}, \cdots, \mathbf{H}_{M, m, k}\right\}
\end{equation}
\begin{equation}
	\mathbf{H}_{m, m, k}=\mathbf{I}_K \otimes \mathbf{h}_{m, m, k}^H
\end{equation}
\begin{equation}
	\mathbf{t}=\left[\mathbf{t}_1^T , \mathbf{t}_2^T , \ldots , 
		\mathbf{t}_M^T\right]^T
\end{equation}
And $\mathbf{s}_{m, k}$ has a one in the $\left(\left( m-1 \right)K+k\right)$-th position and zeros elsewhere.
Leveraging the second order cone programming, 
we can further relax the SINR constraint \eqref{sub1_2}, transforming it into the following set of convex constraints:
\begin{subequations}
	\begin{align}
		\left\|\left[\mathbf{H}_{m, k} \mathbf{t} ; \sigma_n\right]\right\|
		\leq  \left(1+\frac{1}{\Gamma}\right) & \mathrm{real} \left(\mathbf{s}_{m, k}^H \mathbf{H}_{m, k} \mathbf{t}\right), 
		\forall m, k  \label{sub1_31}\\
		\mathrm{imag} \left(\mathbf{s}_{m, k}^H \mathbf{H}_{m, k} \mathbf{t}\right) &= 0, \forall m, k \label{sub1_32}
	\end{align} 
\end{subequations}
Next, the optimization objective can be rewritten as:
\begin{subequations}
	\begin{align}
		\min_{\left\{ \mathbf{t}_{m}, t_m\right\}} &
		\frac{\rho_1}{2} \sum_{m=1}^{M}  \left( \left( q_m + b_m \right)^2 \right. \nonumber \\
		& \left. - 2\left( q_m + b_m \right) \mathbf{t}_{m}^H 
		\mathbf{A}   \mathbf{t}_{m}  
		+  t_m^2 \right) \\ 
		& + \frac{\rho_2}{2} \sum_{m=1}^{M}  \left\| \mathbf{t}_m \! - \!\mathrm{vec}\left( \mathbf{F}_{RF,m}\mathbf{F}_{BB,m} \! - \!
		\mathbf{D}_m \right) \right\|^2  \nonumber\\
		\text{ s.t. } & \mathbf{t}_m^H \mathbf{A} \mathbf{t}_m \leq t_m, \forall m \label{t_m}
	\end{align}  \label{sub1_5}
\end{subequations}
where:
\begin{equation}
	\mathbf{F}_{BB,m} = \left[ \mathbf{f}_{BB,m,1}, \mathbf{f}_{BB,m,2}, \ldots, \mathbf{f}_{BB,m,K}\right] \label{F_BB}
\end{equation}
\begin{equation}
	\mathbf{D}_m = \left[ \mathbf{d}_{m,1}, \mathbf{d}_{m,2}, \ldots, \mathbf{d}_{m,K} \right] \label{D}
\end{equation}
\begin{equation}
	\mathbf{A} = \mathbf{I}_K \otimes 
		\left(  \mathbf{a}^*\left( \theta_m \right) \mathbf{a}^T\left( \theta_m \right) \right) \succeq 0
\end{equation}
Note that we have incorporated the following established fact into the above calculations:
\begin{equation}
	\begin{aligned}
		\mathbf{a}^T  \left( \theta_m \right) \sum_{k=1}^{K} \mathbf{t}_{m,k} \mathbf{t}_{m,k}^H \mathbf{a}^*\left( \theta_m \right)=
		\mathbf{t}_{m}^H   \mathbf{A}  \mathbf{t}_{m}
	\end{aligned}  \label{sub1_1}	
\end{equation}
We can infer, by contradiction, that the constraint \eqref{t_m} is active at the optimum, 
thereby establishing that \eqref{27a} is equivalent to \eqref{sub1_5}.
Despite the absence of a quartic term in the objective function \eqref{sub1_5}, 
the function retains its non-convex nature due to the presence of 
the term $-2\left(q_m+b_m\right) \mathbf{t}_m^H \mathbf{A} \mathbf{t}_m$, 
which exhibits concavity with respect to $\mathbf{t}_m$. 
To tackle this issue, we substitute the concave term with its upper bound, specifically, 
the first-order Taylor expansion at the $i$-th iteration, as illustrated in \eqref{sub1_6}:
\begin{equation}
	\hspace{-0.2cm}\begin{aligned}
		&-2\left(q_m+b_m\right) \mathbf{t}_m^H\mathbf{A} \mathbf{t}_m \\
		&\leq \! - \!4\left(q_m\!+\!b_m\right) \mathrm{Re} \left( \mathbf{t}_m^H\mathbf{A} \mathbf{t}_m^{(i)} \right)
		\!+ \!2\left(q_m\!+\!b_m\right) {\mathbf{t}_m^{(i)}}^H\mathbf{A} \mathbf{t}_m^{(i)}
	\end{aligned}  \label{sub1_6}
\end{equation}
where $\mathbf{t}_m^{(i)}$ is the solution to the subproblem 1 at the $i$-th iteration.


Building on the previous analysis and disregarding any irrelevant terms, 
we can reformulate subproblem 1 at the $\left( i+1 \right)$-th iteration as follows:
\begin{equation}
	\begin{aligned}
		\min_{\left\{ \mathbf{t}_{m}, t_m\right\}} &
		\frac{\rho_1}{2} \sum_{m=1}^{M}  \left(   -   4\left( q_m \! +\! b_m \right) \mathrm{Re} \left( \mathbf{t}_{m}^H \mathbf{A}
		\mathbf{t}_{m}^{(i)}  \right) 	\!+ \!t_m^2 \right) 	\\
		&  + \frac{\rho_2}{2} \sum_{m=1}^{M} \left( \left\| \mathbf{t}_m \right\|^2 \right. \\
		&\left. -2 \mathrm{Re} \left( \mathbf{t}_m^H
		\mathrm{vec}\left( \mathbf{F}_{\mathrm{RF},m}\mathbf{F}_{\mathrm{BB},m} -\mathbf{D}_m \right)  \right) \right)\\
		\text { s.t. }& \eqref{sub1_4}, \eqref{sub1_42}, \eqref{sub1_31},  \eqref{sub1_32} , \eqref{t_m}
		\end{aligned}  \label{sub1_7}
\end{equation}

Following the aforementioned transformations, problem \eqref{sub1} has now been converted 
into a convex optimization problem \eqref{sub1_7} that
can be efficiently solved using the CVX tool, as referenced in \cite{grantCVXMatlabSoftware2014}.

\subsection{Subproblem 2: Update $\left\{q_m\right\}$, $\mu_1$, and $\mu_2$}
The subproblem 2 can be formulated as:
\begin{subequations}
	\begin{align}
		\min_{\left\{ q_m \right\}, \mu_1, \mu_2}  &
		\mu_1+\mu_2+ \frac{\rho_1}{2} \sum_{m=1}^{M} \left| q_m\right. \\
		& \left. - \mathbf{a}^T\left( \theta_m \right) \left( \sum_{k=1}^{K} 
		\mathbf{t}_{m,k}\mathbf{t}_{m,k}^H \right) \mathbf{a}^*\left( \theta_m \right)+b_m \right|^2  \nonumber \\
		\text { s.t. }  &\left[\begin{array}{cc}
			\mathbf{\Lambda Z} \mathbf{\Lambda}^T & \mathbf{e}_i \\
			\mathbf{e}_i^T & \mu_i
		\end{array}\right] \succeq 0, i=1,2 
	\end{align}  \label{sub2}
\end{subequations}
This subproblem is convex and can be efficiently solved using the CVX tool \cite{grantCVXMatlabSoftware2014}.

\subsection{Subproblem 3: Update $\left\{\mathbf{f}_{BB,m,k}\right\}$}
The subproblem 3 can be formulated as:
\begin{equation}
	\begin{aligned}
		\min_{\left\{   \mathbf{F}_{BB,m} \right\} }  &
		\frac{\rho_2}{2} \sum_{m=1}^{M}  \left\| \mathbf{T}_{m} 
		-\mathbf{F}_{RF,m}\mathbf{F}_{BB,m} + \mathbf{D}_{m} \right\|^2   
	\end{aligned}  \label{sub3}
\end{equation}
where
\begin{equation}
	\mathbf{T}_{m}=\left[ \mathbf{t}_{m,1}, \mathbf{t}_{m,2}, \ldots, \mathbf{t}_{m,K} \right]
\end{equation}
Additional, 
$\mathbf{F}_{BB,m}$ and $\mathbf{D}_m$ are defined in equation \eqref{F_BB} and
\eqref{D}, respectively.
This subproblem is a classical least squares (LS) problem, for which we can derive the closed-form solution as:
\begin{equation}
	\begin{aligned}
		\mathbf{F}_{BB, m}=\mathbf{F}_{RF, m}^{\dagger}\left(\mathbf{T}_m+\mathbf{D}_m\right), \forall m
	\end{aligned}  \label{sub3_1}
\end{equation}

\subsection{Subproblem 4: Update $\left\{\mathbf{F}_{RF,m}\right\}$}
Similar as the subproblem 3, the subproblem 4 can be formulated as:
\begin{equation}
	\begin{aligned}
		\min _{\left\{\mathbf{F}_{RF, m}\right\}}& \frac{\rho_{2}}{2}  \sum_{m=1}^M  
		\left\|\mathbf{T}_m-\mathbf{F}_{RF, m} \mathbf{F}_{BB, m}+\mathbf{D}_m\right\|^2 \\
		\text{s.t.} &\left|\mathbf{F}_{RF, m}(i, j)\right|=1, \forall i,  j  
	\end{aligned}  \label{sub4}
\end{equation}
Despite the non-convex nature of this subproblem, stemming from the constant modulus constraints, 
it can be effectively addressed using the Riemannian manifold optimization (MO) algorithm, 
as elaborated in \cite{chengQoSAwareHybridBeamforming2022}.
The Euclidean gradient  of the objective function in \eqref{sub4}, 
as utilized in the Riemannian MO algorithm, is as follows:
\begin{equation}
	\begin{aligned}
		\nabla f\left(\mathbf{F}_{RF, m}\right)  &=  -   2\left(\mathbf{T}_m + \mathbf{D}_m \right. \\
		&\left. - \mathbf{F}_{RF, m} 
		\mathbf{F}_{BB, m}\right) \mathbf{F}_{BB, m}^H, \forall m
	\end{aligned}  \label{sub4_1}
\end{equation}

\subsection{Subproblem 5: Update $\left\{\mathbf{d}_{m,k}\right\}$ and $\left\{b_m\right\}$}
As per \cite{boydDistributedOptimizationStatistical2010}, 
during the $\left( i+1 \right)$ iteration, 
the auxiliary variables $\left\{\mathbf{d}_{m,k}\right\}$ and $\left\{b_m\right\}$ can be updated using 
the subsequent closed-form solutions:
\begin{equation}
	\begin{aligned}
		\mathbf{d}_{m,k} = \mathbf{t}_{m,k} - \mathbf{F}_{RF,m}\mathbf{f}_{BB,m,k} +
		\mathbf{d}_{m,k}^{\left( i \right)} , \forall m, k
	\end{aligned}  \label{sub5_1}
\end{equation}
\begin{equation}
	\begin{aligned}
		b_m = q_m - & \mathbf{a}^T\left( \theta_m \right) \left( \sum_{k=1}^{K} 
		\mathbf{t}_{m,k}\mathbf{t}_{m,k}^H \right) \mathbf{a}^*\left( \theta_m \right) \\
		& + b_m^{\left( i \right)}, \forall m
	\end{aligned}  \label{sub5_2}
\end{equation}
where $\mathbf{d}_{m,k}^{\left( i \right)}$ and $b_m^{\left( i \right)}$ are 
the solutions to the subproblem 5 at the $i$-th iteration, respectively.


The proposed ADMM-based hybrid beamforming algorithm cycles through 
subproblems 1-5 until a specified stopping criterion is satisfied. 
This could be either reaching the maximum number of iterations, denoted as $I$,
or meeting the convergence threshold $\epsilon_D$ and $\epsilon_b$. 
A detailed depiction of the algorithm is provided in Algorithm 1.

\begin{algorithm}[!t]
	\caption{ADMM based Hybrid Beamforming Algorithm}
	\begin{algorithmic}[1]
		\STATE \textbf{Initialization:} Set initial variables $\rho_1$, $\rho_2$, $\left\{\mathbf{d}_{m,k}^{\left( 0 \right)}\right\}$, 
		$\left\{b_m^{\left( 0 \right)}\right\}$, $\left\{\mathbf{t}_{m,k}^{\left( 0 \right)}\right\}$, 
		$\left\{\mathbf{F}_{RF,m}^{\left( 0 \right)}\right\}$, 
		$\left\{\mathbf{f}_{BB,m,k}^{\left( 0 \right)}\right\}$, 
		$\left\{q_m^{\left( 0 \right)}\right\}$, $\mu_1^{\left( 0 \right)}$ and $\mu_2^{\left( 0 \right)}$. 
		\STATE Set $i=1$. 
		\STATE \textbf{repeat}
		\STATE \hspace{0.5cm} Update $\left\{\mathbf{t}_{m,k}^{\left(i\right)}\right\}$ by solving \eqref{sub1_7}.
		\STATE \hspace{0.5cm} Update $\left\{q_m^{\left(i\right)}\right\}$, $\mu_1^{\left(i\right)}$, and 
								$\mu_2^{\left(i\right)}$ by solving \eqref{sub2}.
		\STATE \hspace{0.5cm} Update $\left\{\mathbf{f}_{BB,m,k}^{\left(i\right)}\right\}$ using \eqref{sub3_1}.
		\STATE \hspace{0.5cm} Update $\left\{\mathbf{F}_{RF,m}^{\left(i\right)}\right\}$ by solving \eqref{sub4}.
		\STATE \hspace{0.5cm} Update $\left\{\mathbf{d}_{m,k}^{\left(i\right)}\right\}$ and 
								$\left\{b_m^{\left(i\right)}\right\}$ using \eqref{sub5_1} and \eqref{sub5_2}.
		\STATE \hspace{0.5cm} $i=i+1$.
		\STATE \textbf{until} $i>I$, or $\sum_{m=1}^{M}\left\| 
			\mathbf{T}_{m}^{\left( i \right)} - \mathbf{F}_{RF,m}^{\left( i \right)}
			\mathbf{F}_{BB,m}^{\left( i \right)} \right\|^2 \leq \epsilon_D$ and
			$\sum_{m=1}^{M}\left| q_m^{\left( i \right)} - \mathbf{a}^T\left( \theta_m \right)
			\mathbf{T}_{m}^{\left( i \right)}\mathbf{T}_{m}^{\left( i \right)H} 
			\mathbf{a}^*\left( \theta_m \right)  \right|^2 \leq \epsilon_b$.
		\STATE \textbf{Output:} $\left\{\mathbf{F}_{RF,m}\right\}$ and $\left\{\mathbf{f}_{BB,m,k}\right\}$.
	\end{algorithmic}
\end{algorithm}

We now proceed to examine the complexity of the proposed hybrid beamforming algorithm. 
The complexities associated with solving \eqref{sub1_7} and \eqref{sub2} are 
$\mathcal{O}\left( \ln(1/\epsilon_1) M^{3.5} K^{3.5}N_t^{3} \right)$ 
and $\mathcal{O}\left( \ln(1/\epsilon_2) M^{3.5} \right)$, respectively, 
where $\epsilon_1$ and $\epsilon_2$ represent the solution accuracies for Subproblems 1 and 2, respectively. 
The complexity of solving \eqref{sub4} primarily arises from the computation of the Euclidean gradient, 
which is $\mathcal{O}\left( I_{1} M K N_t N_{RF} \right)$, with $I_{1}$ denoting the number of 
iterations needed for MO convergence. The complexity of calculating \eqref{sub3_1}, \eqref{sub5_1} and \eqref{sub5_2} are
$\mathcal{O}\left( M N_{RF}^2 N_t \right)$, $M K N_t N_{RF}$ and $M K N_t^2$, respectively. Hence, the total complexity of 
the proposed hybrid beamforming algorithm is 
$\mathcal{O}\left( I_0 \left( \ln(1/\epsilon_1) M^{3.5} K^{3.5}N_t^{3}\!+\! \ln(1/\epsilon_2) 
M^{3.5} \! + \! I_{1} M K N_t N_{RF} \right. \right.$
$\left.\left.+ M N_{RF}^2 N_t + M K N_t N_{RF} + M K N_t^2 \right)\right)$, 
where $I_0$ is the number of iterations required for ADMM convergence.


==> subText/socp.tex <==
\section{Coordinated Beamforming Algorithm Based on SCA}
To overcome the non-convexity challenges of problem \eqref{eq:problem_lmi}, 
particularly arising from the SINR constraint \eqref{p2} and the nonlinear 
matrix inequality \eqref{nlmi}, we present a sub-optimal coordinated beamforming algorithm 
that employs the SCA technique. This approach  presents a lower complexity alternative to
the SDP-based algorithm. It accomplishes this by iteratively 
solving a sequence of convex approximations, each step bringing us 
closer to the solution of the original problem.

To begin, we introduce a set of auxiliary variables, $\left\{q_{m}\right\}$,
to reformulate the equation \eqref{J_ele} as follows:
\begin{equation}
	\begin{aligned}
		J(\tau_{m,n},\tau_{m,n})  = \frac{8\pi^2 L \beta^2 \left| \varepsilon_{m,n} \right|^2 q_m}
		{\sigma_{\mathrm{s}}^2}  
	\end{aligned}  \label{J_ele3}
\end{equation}
By introducing the auxiliary variables,
we can get the following reformulation of the problem \eqref{eq:problem_lmi}:
\begin{subequations}
	\begin{align}
		\mathop{\text{minimize}}\limits_{{\left\{\mathbf{f}_{m, k}\right\}, \mu_1, \mu_2, \left\{q_{m}\right\}}} \quad &  \mu_1+\mu_2 \\
		\text {subject to} \quad \quad \  &  \eqref{p1}, \eqref{p3}, \eqref{p2}  \\
		& \left[\begin{array}{cc}
			\mathbf{\Lambda Z} \mathbf{\Lambda}^T & \mathbf{e}_i \\
			\mathbf{e}_i^T & \mu_i
				\end{array}\right] \succeq 0, i=1,2 \\
		& \begin{aligned}
			q_m & \leq \mathbf{a}^T\left(\theta_m\right) 
			\left( 
			\sum_{k=1}^{K}\mathbf{f}_{m,k}\mathbf{f}_{m,k}^H \right) \\
			& \times \mathbf{a}^{*}\left(\theta_m\right), \forall m
		\end{aligned} \label{q}
	\end{align}
	\label{eq:problem_lmi2}%
\end{subequations}
Comparing the problem \eqref{eq:problem_lmi2} with the original problem \eqref{eq:problem_lmi},
we can get the following Theorem:
\begin{theorem}
	The problem \eqref{eq:problem_lmi2} is equivalent to the original problem \eqref{eq:problem_lmi}.
\end{theorem}
\begin{IEEEproof}
	Please refer to Appendix C.
\end{IEEEproof}

Transforming problem \eqref{eq:problem_lmi} into its reformulated version \eqref{eq:problem_lmi2} 
makes the constraints \eqref{nlmi} linear, thereby simplifying the solution process. 
However, the SINR constraint \eqref{p2} retains its non-convex nature, 
and the introduction of the new constraint \eqref{q} adds another layer of non-convexity to the problem.
To address these challenges, 
we define $\left\{\mathbf{f}_{m}\right\}$ as the following vector:
\begin{equation}
	\mathbf{f}_{m} = \left[ \mathbf{f}_{m,1}^T,\mathbf{f}_{m,2}^T, \ldots, 
		\mathbf{f}_{m,K}^T \right]^T, \forall m
\end{equation}

Following the definition above, we can accordingly reformulate 
the constraints for total power and per-BS power as:
\begin{subequations}
	\begin{align}
		\sum_{m=1}^{M}  \mathbf{f}_{m}^H  \mathbf{f}_{m}  &\leq P  \label{sub1_4} \\
		\mathbf{f}_{m}^H  \mathbf{f}_{m}  & \leq P_{m}, \forall m \label{sub1_42}
	\end{align} 
\end{subequations}

Correspondingly, the SINR constraint can be rewritten as:
\begin{equation}
	\begin{aligned}
		\left\|\left[\mathbf{H}_{m, k} \mathbf{f} ; \sigma_{\mathrm{n}}\right]\right\|^2
		\leq\left(1+\frac{1}{\Gamma}\right)\left|\mathbf{s}_{k}^T \mathbf{H}_{m,m, k}
		\mathbf{f}_m\right|^2, \forall m, k
	\end{aligned} \label{sub1_2}
\end{equation}
Here, we define $\mathbf{f}$, $\mathbf{H}_{i,m, k}$, and $\mathbf{H}_{m, k}$   as:
\begin{subequations}
	\begin{align}
		\hspace{-0.1cm}\mathbf{f}& =\left[\mathbf{f}_1^T , \mathbf{f}_2^T , \ldots, 
			\mathbf{f}_M^T\right]^T \\
			\hspace{-0.1cm}\mathbf{H}_{i,m, k} & = \mathbf{I}_K \otimes \mathbf{h}_{i, m, k}^H, \forall i, m, k \\
			&\begin{aligned}
				\hspace{-0.81cm}\mathbf{H}_{m, k} =\operatorname{diag}&\left(\mathbf{H}_{1, m, k}, 
				\mathbf{H}_{2, m, k}, \right. \\
				& \left. \cdots, \mathbf{H}_{M, m, k}\right), \forall m, k 
			\end{aligned}
	\end{align}
\end{subequations}
Besides, $\mathbf{s}_{k}$ is a vector with dimension $K$, which 
has a one in the $k$-th 
position and zeros elsewhere.
If $\mathbf{f}_{m,k}$ is an optimal solution,
then $\mathbf{f}_{m,k}e^{\jmath \varsigma_{m,k}}$
is also an optimal solution, where $\varsigma_{m,k}$ is an arbitrary phase.
Therefore, we can assume that $\mathbf{s}_{k}^T \mathbf{H}_{m,m, k} \mathbf{f}_m$ is a real number.
With this assumption,
the non-convex SINR constraint \eqref{sub1_2} is equivalent to the following convex constraint:
\begin{equation}
	\begin{aligned}
		\left\|\left[\mathbf{H}_{m, k} \mathbf{f} ; \sigma_n\right]\right\|
		\leq  \left(1+\frac{1}{\Gamma}\right)   \mathrm{Re} \left(\mathbf{s}_{k}^T 
		\mathbf{H}_{m,m, k} \mathbf{f}_m\right), 
		\forall m, k  \label{sub1_31}
	\end{aligned} 
\end{equation}



%\begin{equation}
%	\mathrm{Imag} \left(\mathbf{s}_{m, k}^H \mathbf{H}_{m, k} \mathbf{f}\right)  = 0, \forall m, k \label{sub1_32}
%\end{equation}
%Note that the constraints \eqref{sub1_31} and \eqref{sub1_32} are not totally
%equivalent to the original SINR constraint \eqref{sub1_2}, but they are convex 
%and can be used as a stringent approximation to the original constraint.


Additionally, the constraint \eqref{q} can be rewritten as:
\begin{equation}
	\begin{aligned}
		\mathbf{f}_{m}^H   \mathbf{A}  \mathbf{f}_{m} \geq q_m, \forall m
	\end{aligned}  \label{sub1_1}	
\end{equation}
Here, we define $\mathbf{A}$ as:
\begin{equation}
	\mathbf{A} = \mathbf{I}_K \otimes 
		\left(  \mathbf{a}^*\left( \theta_m \right) \mathbf{a}^T\left( \theta_m \right) \right) \succeq 0
\end{equation}
The constraint \eqref{sub1_1} is still non-convex,
but the SCA technique can be employed to replace 
it with a sequence of lower bound approximations, such as 
its first-order Taylor expansion,  in a linear form.
Specifically, given optimal solutions $\left\{\mathbf{f}_{m}^{(t)}\right\}$ at the $t$-th iteration,
the constraint \eqref{sub1_1} at the $\left( t+1 \right)$-th iteration can be approximated as:
\begin{equation}
	\begin{aligned}
		2\operatorname{Re}\left( \mathbf{f}_{m}^H   \mathbf{A}  \mathbf{f}_{m}^{(t)} \right)
		- \left(\mathbf{f}_{m}^{(t)}\right)^H   \mathbf{A}  \mathbf{f}_{m}^{(t)}  \geq q_m, \forall m
	\end{aligned}  \label{sub1_1_2}
\end{equation}
which is a linear constraint and can be efficiently processed.

Building on the above analysis and reformulations,
the problem \eqref{eq:problem_lmi2}
at the $\left( t+1 \right)$-th iteration can be formulated as:
\begin{subequations}
	\begin{align}
		\mathop{\text{minimize}}\limits_{{\left\{\mathbf{f}_{m, k}\right\}, \mu_1, \mu_2, \left\{q_{m}\right\}}} \quad &   \mu_1+\mu_2 \\
		\text {subject to} \quad \quad \  &  \eqref{sub1_4}, \eqref{sub1_42}, \eqref{sub1_31}, \eqref{sub1_1_2} 
	\end{align}
	\label{eq:problem_lmi3}%
\end{subequations}
The problem \eqref{eq:problem_lmi3} is a second order cone programming (SOCP) problem, 
which can be more efficiently solved than the SDP problem \eqref{eq:problem_eq}.
By iteratively solving a sequence of the SOCP problem \eqref{eq:problem_lmi3},
we can obtain the sub-optimal solution to the original problem \eqref{eq:problem_lmi}.
The proposed beamforming algorithm based on SCA is summarized in Algorithm \ref{alg:SCA}.
\begin{algorithm}[t]
	\caption{Coordinated Beamforming Algorithm Based on SCA}
	\label{alg:SCA}
	\begin{algorithmic}[1]
		\STATE \textbf{Initialization:} Set $t=0$, and initialize $\left\{\mathbf{f}_{m}^{(0)}\right\}$.
		\REPEAT
		\STATE \textbf{Step 1:} Given $\left\{\mathbf{f}_{m, k}^{(t)}\right\}$, solve the SOCP problem \eqref{eq:problem_lmi3} 
			to obtain $\left\{\mathbf{f}_{m}^{(t+1)}\right\}$, $\mu_1$, $\mu_2$, and $\left\{q_m\right\}$.
		\STATE \textbf{Step 2:} Set $t=t+1$.
		\UNTIL{the predefined stopping criterion is satisfied.}
		\STATE \textbf{Output:} $\left\{\mathbf{f}_{m}^{(t)}\right\}$.
	\end{algorithmic}
\end{algorithm}

We now delve into the complexity analysis of the proposed beamforming algorithm based on SCA.
The problem defined by \eqref{eq:problem_lmi3} is a SOCP problem.
It can be solved with a computational complexity of
$\mathcal{O}\left(\ln(1/\epsilon)\left( M^{2.5}K^{2.5}N_{\mathrm{t}}^{3} +  
M^{3.5}K^{3.5}N_{\mathrm{t}} \right)\right)$  
\cite{wangPartiallyConnectedHybridBeamforming2022}, given
a same solution accuracy $\epsilon > 0$ as the SDP problem \eqref{eq:problem_eq}.
Assuming that the SCA method needs to be iterated $I_2$ times to converge,
the overall complexity of the proposed beamforming algorithm based on SCA is about
$\mathcal{O}\left(\ln(1/\epsilon)\left( M^{2.5}K^{2.5}N_{\mathrm{t}}^{3} +  
M^{3.5}K^{3.5}N_{\mathrm{t}} \right)I_2\right)$.
Comparing the complexity of the SCA-based algorithm with the SDP-based algorithm,
we can see that the SCA-based algorithm has a lower computational complexity.
This is mainly due to the fact that the SOCP problem is more efficient to solve than the SDP problem.







==> subText/tmp1.tex <==
Typically, the obtained solution $\mathbf{F}_{m,k}^{\star}$ will not be rank-one, suggesting  that an
approximating method, such as Gaussian randomization method \cite{Luo2006}, 
is required to extract the beamforming vectors $\mathbf{f}_{m,k}^{\star}$ 
from $\mathbf{F}_{m,k}^{\star}$. 
Specifically, the eigenvalue decomposition of $\mathbf{F}_{m,k}^{\star}$ is expressed as:
\begin{equation}
	\mathbf{F}_{m,k}^{\star} = \mathbf{U}_{m,k} \mathbf{\Sigma}_{m,k} \mathbf{U}_{m,k}^H
\end{equation}
where $\mathbf{U}_{m,k}$ is the unitary matrix and $\mathbf{\Sigma}_{m,k}$ is the diagonal matrix. 
Following this, a vector $\mathbf{v}_{m,k}$ is generated as:
\begin{equation}
	\mathbf{v}_{m,k} = \mathbf{U}_{m,k} \mathbf{\Sigma}_{m,k}^{\frac{1}{2}} \mathbf{z}_{m,k}
\end{equation}
where $\mathbf{z}_{m,k}$ is a
random vector with independent and identically distributed standard normal distribution. 
Subsequently, 
scaling factors $\left\{\alpha_{m,k}\right\}\geq 0$ are introduced, and  
the optimization variables $\left\{\mathbf{F}_{m,k}\right\}$ are replaced with 
$\left\{\alpha_{m,k}\mathbf{v}_{m,k}\mathbf{v}_{m,k}^H\right\}$.
Consequently, the equation \eqref{J_ele} is reformulated as:
\begin{equation}
    \begin{aligned}
        J(\tau_{m,n},\tau_{m,n}) & = \frac{8\pi^2 L \beta^2 \left| \varepsilon_{m,n} \right|^2}{\sigma_{\mathrm{s}}^2}
		\\ & \times  
        \left( 
        \sum_{k=1}^{K}\alpha_{m,k} \left|\mathbf{a}^T\left(\theta_m\right) \mathbf{v}_{m,k} \right|^2 \right)  
    \end{aligned}  \label{J_ele5}
\end{equation}
The problem \eqref{eq:problem_eq} is then reformulated as:
\begin{subequations}
    \begin{align}
        &\min_{\left\{\alpha_{m, k}\right\}, \mu_1, \mu_2} \mu_1+\mu_2 \\
        \text { s.t. } &  \operatorname{tr}\left(\sum_{m=1}^M\sum_{k=1}^K 
		\alpha_{m,k}\mathbf{v}_{m,k}\mathbf{v}_{m,k}^H \right)
		\leq P   \\
		&\operatorname{tr}\left(\sum_{k=1}^K \alpha_{m,k}\mathbf{v}_{m,k}\mathbf{v}_{m,k}^H \right)
		\leq P_m, \forall m   \\
        & \begin{aligned} 
							& \alpha_{m,k} \left| \mathbf{h}_{m, m, k}^{H} \mathbf{v}_{m,k} \right|^2 \geq \\ 
							& \Gamma \left( \sum_{i=1}^{M} \sum_{j=1,j\neq k}^K \alpha_{i,j} \left|\mathbf{h}_{i, m, k}^H 
							\mathbf{v}_{i,j}\right|^2 +
							\sigma_n^2 \right) , \forall m, k
						\end{aligned}  \\
		& \left[\begin{array}{cc}
			\mathbf{\Lambda Z} \mathbf{\Lambda}^T & \mathbf{e}_i \\
			\mathbf{e}_i^T & \mu_i
		\end{array}\right] \succeq 0, i=1,2  \\
		&  \alpha_{m,k} \geq 0, \forall m, k 
    \end{align}
    \label{eq:problem_eq2}%
\end{subequations}
It is a convex problem and can be solved efficiently.
The optimal scaling factor, denoted as $\alpha_{m,k}^{\star}$,
allows for the derivation of the beamforming vector $\mathbf{f}_{m,k}^{\star}$ as:
\begin{equation}
	\mathbf{f}_{m,k}^{\star} = \alpha_{m,k}^{\star}\mathbf{v}_{m,k}
\end{equation}
